The Excited Spin State of 1I/2017 U1 `Oumuamua

We show that `Oumuamua's excited spin could be in a high energy LAM state, which implies that its shape could be far from the highly elongated shape found in previous studies. CLEAN and ANOVA algorithms are used to analyze `Oumuamua's lightcurve using 818 observations over 29.3~days. Two fundamental periodicities are found at frequencies (2.77$\pm$0.11) and (6.42$\pm$0.18)~cycles/day, corresponding to (8.67$\pm$0.34)~h and (3.74$\pm$0.11)~h, respectively. The phased data show that the lightcurve does not repeat in a simple manner, but approximately shows a double minimum at 2.77~cycles/day and a single minimum at 6.42~cycles/day. This is characteristic of an excited spin state. `Oumuamua could be spinning in either the long (LAM) or short (SAM) axis mode. For both, the long axis precesses around the total angular momentum vector with an average period of (8.67$\pm$0.34)~h. For the three LAMs we have found, the possible rotation periods around the long axis are 6.58, 13.15, or 54.48~h, with 54.48~h being the most likely. `Oumuamua may also be nutating with respective periods of half of these values. We have also found two possible SAM states where `Oumuamua oscillates around the long axis with possible periods at 13.15 and 54.48~h, the latter as the most likely. In this case any nutation will occur with the same periods. Determination of the spin state, the amplitude of the nutation, the direction of the TAMV, and the average total spin period may be possible with a direct model fit to the lightcurve. We find that `Oumuamua is "cigar-shaped"', if close to its lowest rotational energy, and an extremely oblate spheroid if close to its highest energy state for its total angular momentum.

==> Tab-Data.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lcccccccccl}
%\tabletypesize{\small}
\tablecaption{Observing Geometry and Photometry \label{tab:data}}
\tablehead{
\colhead{UTDate                    } &
\colhead{JD\tablenotemark{a}       } &
\colhead{$r$\tablenotemark{b}      } &
\colhead{$\Delta$\tablenotemark{b} } &
\colhead{$\alpha$\tablenotemark{b} } &
\colhead{TA\tablenotemark{c}       } &
\colhead{Filt                      } &
\colhead{\# Images                 } &
\colhead{mag$\pm$$\sigma$          } &
\colhead{r$_{mag}$$\pm$$\sigma$\tablenotemark{d}} &
\colhead{Color/Comment}
}
\startdata
\multicolumn{11}{l}{\bf PanSTARRS1 data}\\
2010/06/04 & 5352.10123	& 28.665 & 28.754 & 2.017 & -151.16 & i$_{p1}$ &  2 & $<$21.0$\pm$0.3   & $<$21.2$\pm$0.3  & Limiting mag \\
2012/08/07 & 6146.81325	& 25.061 & 25.146 & 2.306 & -149.01 & r$_{p1}$ &  2 & $<$21.8$\pm$0.3   & $<$21.8$\pm$0.3  & Limiting mag \\
2014/06/14 & 6821.46247 & 21.802 & 21.829 & 2.666 & -146.54 & i$_{p1}$ &  3 & $<$21.0$\pm$0.3   & $<$21.2$\pm$0.3  & Limiting mag \\ 
2014/06/13 & 6822.51886 & 21.797 & 21.824 & 2.667 & -146.54 & i$_{p1}$ &  3 & $<$20.7$\pm$0.3   & $<$20.9$\pm$0.3  & Limiting mag \\
2014/07/05 & 6844.27742 & 21.688 & 21.729 & 2.681 & -146.45 & i$_{p1}$ &  2 & $<$20.8$\pm$0.3   & $<$21.0$\pm$0.3  & Limiting mag \\ 
2014/03/20 & 6737.07683 & 22.221 & 22.202 & 2.569 & -146.88 & r$_{p1}$ &  2 &    20.67$\pm$0.30 & 20.67$\pm$0.30 & \\
2014/09/08 & 6908.76850 & 21.364 & 21.430 & 2.692 & -146.17 & i$_{p1}$ &  4 &    20.60$\pm$0.05 & 20.77$\pm$0.05 & \\
2015/05/06 & 7149.01152 & 20.138 & 20.122 & 2.871 & -145.09 & i$_{p1}$ &  4 &    20.10$\pm$0.04 & 20.28$\pm$0.04 & \\
2015/05/07 & 7150.00904 & 20.133 & 20.117 & 2.872 & -145.08 & i$_{p1}$ &  4 &    20.27$\pm$0.05 & 20.45$\pm$0.05 & \\
2016/05/27 & 7536.02124 & 18.088 & 18.052 & 3.211 & -143.07 & r$_{p1}$ &  4 &    19.53$\pm$0.04 & 19.53$\pm$0.04 & \\
2016/06/19 & 7558.88673 & 17.963 & 17.938 & 3.242 & -142.94 & i$_{p1}$ &  3 &    19.37$\pm$0.08 & 19.54$\pm$0.08 & \\
2016/06/21 & 7560.93624 & 17.952 & 17.928 & 3.245 & -142.93 & i$_{p1}$ &  2 &    19.37$\pm$0.06 & 19.54$\pm$0.06 & \\
2016/07/18 & 7587.88946 & 17.805 & 17.803 & 3.270 & -142.77 & i$_{p1}$ &  4 &    19.53$\pm$0.05 & 19.71$\pm$0.05 & \\
2017/04/10 & 7854.05173 & 16.322 & 16.280 & 3.519 & -141.06 & i$_{p1}$ &  4 &    19.19$\pm$0.07 & 19.36$\pm$0.07 & \\
2017/05/21 & 7894.91140 & 16.089 & 16.019 & 3.604 & -140.77 & w$_{p1}$ &  4 &    19.45$\pm$0.03 & 19.39$\pm$0.03 & Discovery \\
2017/06/16 & 7920.97821 & 15.940 & 15.874 & 3.651 & -140.59 & i$_{p1}$ &  4 &    18.85$\pm$0.04 & 19.02$\pm$0.04 & \\
2017/06/25 & 7929.91675 & 15.888 & 15.828 & 3.666 & -140.52 & w$_{p1}$ &  4 &    19.19$\pm$0.03 & 19.13$\pm$0.03 & \\
2017/08/06 & 7971.88255 & 15.646 & 15.638 & 3.715 & -140.21 & i$_{p1}$ &  4 &    18.94$\pm$0.05 & 19.11$\pm$0.05 & \\
2017/08/17 & 7982.77565 & 15.583 & 15.594 & 3.721 & -140.13 & w$_{p1}$ &  4 &    19.02$\pm$0.01 & 18.97$\pm$0.02 & \\
2017/08/30 & 7995.76736 & 15.508 & 15.542 & 3.725 & -140.03 & i$_{p1}$ &  4 &    18.78$\pm$0.04 & 18.96$\pm$0.04 & \\
2017/09/07 & 8003.77876 & 15.461 & 15.511 & 3.724 & -139.96 & i$_{p1}$ &  4 &    18.72$\pm$0.04 & 18.90$\pm$0.04 & \\
2017/06/16 & 7920.95557 & 15.940 & 15.874 & 3.651 & -140.59 & r$_{p1}$ &  4 &    18.96$\pm$0.06 & 19.14$\pm$0.06 & \\
2017/07/05 & 7939.88379 & 15.831 & 15.779 & 3.681 & -140.45 & r$_{p1}$ &  2 &    18.94$\pm$0.14 & 19.11$\pm$0.14 & \\
2017/07/07 & 7941.90196 & 15.819 & 15.770 & 3.684 & -140.43 & r$_{p1}$ &  4 &    19.24$\pm$0.11 & 19.41$\pm$0.11 & \\
2017/07/15 & 7949.87944 & 15.773 & 15.733 & 3.694 & -140.37 & r$_{p1}$ &  4 &    18.82$\pm$0.06 & 19.00$\pm$0.06 & \\
2017/07/17 & 7951.90526 & 15.762 & 15.724 & 3.696 & -140.36 & r$_{p1}$ &  4 &    19.15$\pm$0.20 & 19.33$\pm$0.20 & \\
\hline
\multicolumn{11}{l}{\bf CFHT Archival data from CADC} \\
2013/05/12 & 6424.61132 & 23.744 & 23.767 & 2.436 & -148.07 & u        &  7 &    23.09$\pm$0.17 & 20.76$\pm$0.23 & \\
\hline
\multicolumn{10}{l}{\bf CFHT new data} \\
2017/05/24 & 7898.05595 & 16.071 & 16.000 & 3.610 & -140.75 & w        &  1 &    19.292$\pm$0.007 & 19.237$\pm$0.007 & \\
2017/05/28 & 7901.92345 & 16.049 & 15.978 & 3.617 & -140.72 & g        &  1 &    19.673$\pm$0.015 & & \\
2017/05/28 & 7901.92345 & 16.049 & 15.978 & 3.617 & -140.72 & r        &  1 &    19.155$\pm$0.015 & 19.155$\pm$0.015 & (g-r) = 0.52$\pm$0.02 \\
2017/06/24 & 7928.97060 & 15.894 & 15.833 & 3.665 & -140.53 & g        &  1 &    19.539$\pm$0.012 & & \\
2017/06/24 & 7928.97049 & 15.894 & 15.833 & 3.665 & -140.53 & r        &  1 &    19.067$\pm$0.013 & 19.067$\pm$0.013 & (g-r) = 0.47$\pm$0.02 \\
2017/07/16 & 7950.83854 & 15.768 & 15.729 & 3.695 & -140.37 & r        & 12 &    19.081$\pm$0.004 & 19.081$\pm$0.004 & \\
2017/07/25 & 7990.80063 & 15.768 & 15.729 & 3.695 & -140.37 & g        &  1 &    19.567$\pm$0.011 & & (g-r) = 0.56$\pm$0.02 \\
2017/07/25 & 7990.80285 & 15.768 & 15.729 & 3.695 & -140.37 & r        &  1 &    19.007$\pm$0.012 & 19.007$\pm$0.012 & \\
2017/07/26 & 7991.80022 & 15.537 & 15.562 & 3.724 & -140.06 & u        &  2 &    21.260$\pm$0.054 & & (u-r) = 2.33$\pm$0.06 \\
2017/07/26 & 7991.80602 & 15.531 & 15.558 & 3.724 & -140.06 & g        &  1 &    19.513$\pm$0.013 & & (g-r) = 0.59$\pm$0.02 \\
2017/07/26 & 7991.80407 & 15.537 & 15.562 & 3.724 & -140.06 & r        &  3 &    18.927$\pm$0.008 & 18.927$\pm$0.008 & \\
2017/07/26 & 7991.80889 & 15.531 & 15.558 & 3.724 & -140.06 & i        &  2 &    18.758$\pm$0.013 & & (r-i)\hspace{0.1cm} = 0.17$\pm$0.02 \\
2017/09/14 & 8010.74649	& 15.421 & 15.483 & 3.723 & -139.91 & g	       &  4 &    19.483$\pm$0.005 & & (g-r) = 0.55$\pm$0.01 \\
2017/09/14 & 8010.74282	& 15.421 & 15.483 & 3.723 & -139.91 & r	       &  2 &    18.932$\pm$0.009 & 18.932$\pm$0.009 & \\
2017/09/14 & 8010.74230	& 15.421 & 15.483 & 3.723 & -139.91 & i	       &  6 &    18.761$\pm$0.008 & & (r-i)\hspace{0.1cm} = 0.17$\pm$0.01 \\
2017/09/14 & 8010.75793	& 15.421 & 15.483 & 3.723 & -139.91 & z	       &  4 &    18.721$\pm$0.024 & & (r-z) = 0.21$\pm$0.03 \\
2017/09/15 & 8011.72479	& 15.415 & 15.479 & 3.723 & -139.90 & u	       &  3 &    20.995$\pm$0.039 & & (u-r) = 2.12$\pm$0.04 \\
2017/09/15 & 8011.74031	& 15.415 & 15.479 & 3.723 & -139.90 & g	       &  5 &    19.413$\pm$0.004 & & (g-r) = 0.54$\pm$0.01 \\
2017/09/15 & 8011.75514	& 15.415 & 15.479 & 3.723 & -139.90 & r	       &  2 &    18.873$\pm$0.007 & 18.873$\pm$0.007 & \\
\enddata
\tablenotetext{a}{Julian Date -2450000.0}
\tablenotetext{b}{Heliocentric, geocentric distance (au) and phase angle (deg).}
\tablenotetext{c}{True anomaly (deg), position along orbit, TA at perihelion=0$^{\circ}$}
\tablenotetext{d}{Magnitude and error through 5$''$ radius aperture.}
\tablenotetext{e}{Magnitude and error converted to SDSS $r$ as described in the text}
\end{deluxetable*}
\end{longrotatetable}


==> widetab.tex <==
\begin{longrotatetable}
\begin{deluxetable}{lllrrrrrrll}
\tablecaption{Observable Characteristics of 
Galactic/Magellanic Cloud novae with X-ray observations\label{chartable}}
\tablewidth{700pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{Name} & \colhead{V$_{max}$} & 
\colhead{Date} & \colhead{t$_2$} & 
\colhead{FWHM} & \colhead{E(B-V)} & 
\colhead{N$_H$} & \colhead{Period} & 
\colhead{D} & \colhead{Dust?} & \colhead{RN?} \\ 
\colhead{} & \colhead{(mag)} & \colhead{(JD)} & \colhead{(d)} & 
\colhead{(km s$^{-1}$)} & \colhead{(mag)} & \colhead{(cm$^{-2}$)} &
\colhead{(d)} & \colhead{(kpc)} & \colhead{} & \colhead{}
} 
\startdata
CI Aql & 8.83 (1) & 2451665.5 (1) & 32 (2) & 2300 (3) & 0.8$\pm0.2$ (4) & 1.2e+22 & 0.62 (4) & 6.25$\pm5$ (4) & N & Y \\
{\bf CSS081007} & \nodata & 2454596.5 & \nodata & \nodata & 0.146 & 1.1e+21 & 1.77 (5) & 4.45$\pm1.95$ (6) & \nodata & \nodata \\
GQ Mus & 7.2 (7) & 2445352.5 (7) & 18 (7) & 1000 (8) & 0.45 (9) & 3.8e+21  & 0.059375 (10) & 4.8$\pm1$ (9) & N (7) & \nodata \\
IM Nor & 7.84 (11) & 2452289 (2) & 50 (2) & 1150 (12) & 0.8$\pm0.2$ (4) & 8e+21 & 0.102 (13) & 4.25$\pm3.4$ (4) & N & Y \\
{\bf KT Eri} & 5.42 (14) & 2455150.17 (14) & 6.6 (14) & 3000 (15) & 0.08 (15) & 5.5e+20 & \nodata & 6.5 (15) & N & M \\
{\bf LMC 1995} & 10.7 (16) & 2449778.5 (16) & 15$\pm2$ (17) & \nodata & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
LMC 2000 & 11.45 (18) & 2451737.5 (18) & 9$\pm2$ (19) & 1700 (20) & 0.15 (203) & 7.8e+20  & \nodata & 50 & \nodata & \nodata \\
{\bf LMC 2005} & 11.5 (21) & 2453700.5 (21) & 63 (22) & 900 (23) & 0.15 (203) & 1e+21 & \nodata & 50  & M (24) & \nodata \\
{\bf LMC 2009a} & 10.6 (25) & 2454867.5 (25) & 4$\pm1$  & 3900 (25) & 0.15 (203)  & 5.7e+20 & 1.19 (26) & 50 & N & Y \\
{\bf SMC 2005} & 10.4 (27) & 2453588.5 (27) & \nodata & 3200 (28) & \nodata & 5e+20  & \nodata & 61 & \nodata & \nodata \\
{\bf QY Mus} & 8.1 (29) & 2454739.90 (29) & 60:  & \nodata & 0.71 (30) & 4.2e+21  & \nodata & \nodata & M & \nodata \\
{\bf RS Oph} & 4.5 (31) & 2453779.44 (14) & 7.9 (14) & 3930 (31) & 0.73 (32) & 2.25e+21 & 456 (33) & 1.6$\pm0.3$ (33) & N (34) & Y \\
{\bf U Sco} & 8.05 (35) & 2455224.94 (35) & 1.2 (36) & 7600 (37) & 0.2$\pm0.1$ (4) & 1.2e+21 & 1.23056 (36) & 12$\pm2$ (4) & N & Y \\
{\bf V1047 Cen} & 8.5 (38) & 2453614.5 (39) & 6 (40) & 840 (38) & \nodata & 1.4e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V1065 Cen} & 8.2 (41) & 2454123.5 (41) & 11 (42) & 2700 (43) & 0.5$\pm0.1$ (42) & 3.75e+21 & \nodata & 9.05$\pm2.8$ (42) & Y (42) & \nodata \\
V1187 Sco & 7.4 (44) & 2453220.5 (44) & 7: (45) & 3000 (44) & 1.56 (44) & 8.0e+21 & \nodata & 4.9$\pm0.5$ (44) & N & \nodata \\
{\bf V1188 Sco} & 8.7 (46) & 2453577.5 (46) & 7 (40) & 1730 (47) & \nodata & 5.0e+21  & \nodata & 7.5 (39) & \nodata & \nodata \\
{\bf V1213 Cen} & 8.53 (48) & 2454959.5 (48) & 11$\pm2$ (49) & 2300 (50) & 2.07 (30) & 1.0e+22 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1280 Sco} & 3.79 (51) & 2454147.65 (14) & 21 (52) & 640 (53) & 0.36 (54) & 1.6e+21  & \nodata & 1.6$\pm0.4$ (54) & Y (54) & \nodata \\
{\bf V1281 Sco} & 8.8 (55) & 2454152.21 (55) & 15:& 1800 (56) & 0.7 (57) & 3.2e+21 & \nodata & \nodata & N & \nodata \\
{\bf V1309 Sco} & 7.1 (58) & 2454714.5 (58) & 23$\pm2$ (59) & 670 (60) & 1.2 (30) & 4.0e+21 & \nodata & \nodata & \nodata & \nodata \\
{\bf V1494 Aql} & 3.8 (61) & 2451515.5 (61) & 6.6$\pm0.5$ (61) & 1200 (62) & 0.6 (63) & 3.6e+21  & 0.13467 (64) & 1.6$\pm0.1$ (63) & N & \nodata \\
{\bf V1663 Aql} & 10.5 (65) & 2453531.5 (65) & 17 (66) & 1900 (67) & 2: (68) & 1.6e+22  & \nodata & 8.9$\pm3.6$ (69) & N & \nodata \\
V1974 Cyg & 4.3 (70) & 2448654.5 (70) & 17 (71) & 2000 (19) & 0.36$\pm0.04$ (71) & 2.7e+21  & 0.081263 (70) & 1.8$\pm0.1$ (72) & N & \nodata \\
{\bf V2361 Cyg} & 9.3 (73) & 2453412.5 (73) & 6 (40) & 3200 (74) & 1.2: (75) & 7.0e+21 & \nodata & \nodata & Y (40) & \nodata \\
{\bf V2362 Cyg} & 7.8 (76) & 2453831.5 (76) & 9 (77) & 1850 (78) & 0.575$\pm0.015$ (79) & 4.4e+21  & 0.06577 (80) & 7.75$\pm3$ (77) & Y (81) & \nodata \\
{\bf V2467 Cyg} & 6.7 (82) & 2454176.27 (82) & 7 (83) & 950 (82) & 1.5 (84) & 1.4e+22  & 0.159 (85) & 3.1$\pm0.5$ (86) & M (87) & \nodata \\
{\bf V2468 Cyg} & 7.4 (88) & 2454534.2 (88) & 10: & 1000 (88) & 0.77 (89) & 1.0e+22  & 0.242 (90) & \nodata & N & \nodata \\
{\bf V2491 Cyg} & 7.54 (91) & 2454567.86 (91) & 4.6 (92) & 4860 (93) & 0.43 (94) & 4.7e+21  & 0.09580: (95) & 10.5 (96) & N & M \\
V2487 Oph & 9.5 (97) & 2450979.5 (97) & 6.3 (98) & 10000 (98) & 0.38$\pm0.08$ (98) & 2.0e+21 & \nodata & 27.5$\pm3$ (99) & N (100) & Y (101) \\
{\bf V2540 Oph} & 8.5 (102) & 2452295.5 (102) & \nodata & \nodata & \nodata & 2.3e+21 & 0.284781 (103) & 5.2$\pm0.8$ (103) & N & \nodata \\
V2575 Oph & 11.1 (104) & 2453778.8 (104) & 20: & 560 (104) & 1.4 (105) & 3.3e+21 & \nodata & \nodata & N (105) & \nodata \\
{\bf V2576 Oph} & 9.2 (106) & 2453832.5 (106) & 8: & 1470 (106) & 0.25 (107) & 2.6e+21  & \nodata & \nodata & N & \nodata \\
{\bf V2615 Oph} & 8.52 (108) & 2454187.5 (108) & 26.5 (108) & 800 (109) & 0.9 (108) & 3.1e+21  & \nodata & 3.7$\pm0.2$ (108) & Y (110) & \nodata \\
{\bf V2670 Oph} & 9.9 (111) & 2454613.11 (111) & 15: & 600 (112) & 1.3: (113) & 2.9e+21  & \nodata & \nodata & N (114) & \nodata \\
{\bf V2671 Oph} & 11.1 (115) & 2454617.5 (115) & 8: & 1210 (116) & 2.0 (117) & 3.3e+21  & \nodata & \nodata & M (117) & \nodata \\
{\bf V2672 Oph} & 10.0 (118) & 2455060.02 (118) & 2.3 (119) & 8000 (118) & 1.6$\pm0.1$ (119) & 4.0e+21  & \nodata & 19$\pm2$ (119) & \nodata & M \\
V351 Pup & 6.5 (120) & 2448617.5 (120) & 16 (121) & \nodata & 0.72$\pm0.1$ (122) & 6.2e+21 & 0.1182 (123) & 2.7$\pm0.7$ (122) & N & \nodata \\
{\bf V382 Nor} & 8.9 (124) & 2453447.5 (124) & 12 (40) & 1850 (23) & \nodata & 1.7e+22 & \nodata & \nodata & \nodata & \nodata \\
V382 Vel & 2.85 (125) & 2451320.5 (125) & 4.5 (126) & 2400 (126) & 0.05: (126) & 3.4e+21  & 0.146126 (127) & 1.68$\pm0.3$ (126) & N & \nodata \\
{\bf V407 Cyg} & 6.8 (128) & 2455266.314 (128) & 5.9 (129) & 2760 (129) & 0.5$\pm0.05$ (130) & 8.8e+21 & 15595 (131) & 2.7 (131) & \nodata & Y \\
{\bf V458 Vul} & 8.24 (132) & 2454322.39 (132) & 7 (133) & 1750 (134) & 0.6 (135) & 3.6e+21 & 0.06812255 (136) & 8.5$\pm1.8$ (133) & N (135) & \nodata \\
{\bf V459 Vul} & 7.57 (137) & 2454461.5 (137) & 18 (138) & 910 (139) & 1.0 (140) & 5.5e+21  & \nodata & 3.65$\pm1.35$ (138) & Y (140) & \nodata \\
V4633 Sgr & 7.8 (141) & 2450895.5 (141) & 19$\pm3$ (142) & 1700 (143) & 0.21 (142) & 1.4e+21  & 0.125576 (144) & 8.9$\pm2.5$ (142) & N & \nodata \\
{\bf V4643 Sgr} & 8.07 (145) & 2451965.867 (145) & 4.8 (146) & 4700 (147) & 1.67 (148) & 1.4e+22 & \nodata & 3 (148) & N & \nodata \\
{\bf V4743 Sgr} & 5.0 (149) & 2452537.5 (149) & 9 (150) & 2400 (149) & 0.25 (151) & 1.2e+21 & 0.281 (152) & 3.9$\pm0.3$ (151) & N & \nodata \\
{\bf V4745 Sgr} & 7.41 (153) & 2452747.5 (153) & 8.6 (154) & 1600 (155) & 0.1 (154) & 9.0e+20  & 0.20782 (156) & 14$\pm5$ (154) & \nodata & \nodata \\
{\bf V476 Sct} & 10.3 (157) & 2453643.5 (157) & 15 (158) & \nodata & 1.9 (158) & 1.2e+22  & \nodata & 4$\pm1$ (158) & M (159) & \nodata \\
{\bf V477 Sct} & 9.8 (160) & 2453655.5 (160) & 3 (160) & 2900 (161) & 1.2: (162) & 4e+21  & \nodata & \nodata & M (163) & \nodata \\
{\bf V5114 Sgr} & 8.38 (164) & 2453081.5 (164) & 11 (165) & 2000 (23) & \nodata & 1.5e+21  & \nodata & 7.7$\pm0.7$ (165) & N (166) & \nodata \\
{\bf V5115 Sgr} & 7.7 (167) & 2453459.5 (167) & 7 (40) & 1300 (168) & 0.53 (169) & 2.3e+21  & \nodata & \nodata & N (169) & \nodata \\
{\bf V5116 Sgr} & 8.15 (170) & 2453556.91 (170) & 6.5 (171) & 970 (172) & 0.25 (173) & 1.5e+21 & 0.1238 (171) & 11$\pm3$ (173) & N (174) & \nodata \\
{\bf V5558 Sgr} & 6.53 (175) & 2454291.5 (175) & 125 (176) & 1000 (177) & 0.80 (178) & 1.6e+22  & \nodata & 1.3$\pm0.3$ (176) & N (179) & \nodata \\
{\bf V5579 Sgr} & 5.56 (180) & 2454579.62 (180) & 7: & 1500 (23) & 1.2 (181) & 3.3e+21 & \nodata & \nodata & Y (181) & \nodata \\
{\bf V5583 Sgr} & 7.43 (182) & 2455051.07 (182) & 5: & 2300 (182) & 0.39 (30) & 2.0e+21 & \nodata & 10.5 & \nodata & \nodata \\
{\bf V574 Pup} & 6.93 (183) & 2453332.22 (183) & 13 (184) & 2800 (184) & 0.5$\pm0.1$  & 6.2e+21 & \nodata & 6.5$\pm1$  & M (185) & \nodata \\
{\bf V597 Pup} & 7.0 (186) & 2454418.75 (186) & 3: & 1800 (187) & 0.3 (188) & 5.0e+21  & 0.11119 (189) & \nodata & N (188) & \nodata \\
{\bf V598 Pup} & 3.46 (14) & 2454257.79 (14) & 9$\pm1$ (190) & \nodata & 0.16 (190) & 1.4e+21 & \nodata & 2.95$\pm0.8$ (190) & \nodata & \nodata \\
{\bf V679 Car} & 7.55 (191) & 2454797.77 (191) & 20: & \nodata & \nodata & 1.3e+22  & \nodata & \nodata & \nodata & \nodata \\
{\bf V723 Cas} & 7.1 (192) & 2450069.0 (192) & 263 (2) & 600 (193) & 0.5 (194) & 2.35e+21  & 0.69 (195) & 3.86$\pm0.23$ (196) & N & \nodata \\
V838 Her & 5 (197) & 2448340.5 (197) & 2 (198) & \nodata & 0.5$\pm0.1$ (198) & 2.6e+21  & 0.2975 (199) & 3$\pm1$ (198) & Y (200) & \nodata \\
{\bf XMMSL1 J06} & 12 (201) & 2453643.5 (202) & 8$\pm2$ (202) & \nodata & 0.15 (203) & 8.7e+20 & \nodata & 50 & \nodata & \nodata \\
\enddata
\end{deluxetable}
\end{longrotatetable}

